Simulation of emergence in artificial societies: a practical model-based approach with the EB-DEVS formalism

Modelling and simulation of complex systems is key to exploring and understanding social processes, benefiting from formal mechanisms to derive global-level properties from local-level interactions. In this paper we extend the body of knowledge on formal methods in complex systems by applying EB-DEVS, a novel formalism tailored for the modelling, simulation and live identification of emergent properties. We guide the reader through the implementation of different classical models for varied social systems to introduce good modelling practices and showcase the advantages and limitations of modelling emergence with EB-DEVS, in particular through its live emergence detection capability. This work provides case study-driven evidence for the neatness and compactness of the approach to modelling communication structures that can be explicit or implicit, static or dynamic, with or without multilevel interactions, and with weak or strong emergent behaviour. Throughout examples we show that EB-DEVS permits conceptualising the analysed societies by incorporating emergent behaviour when required, namely by integrating as a macro-level aggregate the Gini index in the Sugarscape model, Fads and Fashion in the Dissemination of Culture model, size-biased degree distribution in a Preferential Attachment model, happiness index in the Segregation model and quarantines in the SIR epidemic model. In each example we discuss the role of communication structures in the development of multilevel simulation models, and illustrate how micro-macro feedback loops enable the modelling of macro-level properties. Our results stress the relevance of multilevel features to support a robust approach in the modelling and simulation of complex systems.

==> axelrod.tex <==
\subsection{Axelrod's model of dissemination of culture}

The Axelrod's model of dissemination of culture model has attracted a lot of attention due its simple rules and its implications in social dynamics. Its interest sits upon the mechanisms it implements for the modeling of cultural assimilation. The model implements two important features, social influence and homophily. It is expected that a social influence model converges to mono-cultural equilibrium. Nevertheless, Axelrod's model presents interesting scenarios where the system drives away from mono-cultural equilibrium towards multi-cultural equilibrium. These scenarios are typically determined by the number of features defining each culture.

\textbf{Model dynamics.} Each agent has a state with two vector variables. A cultural trait array of
size $F$ and each position with values between 1 and $Q$. The agents' state change upon interactions with neighbors. Given an agent and its linked neighbors (assuming an arbitrary topology), the agent selects one neighbor to mix its culture with. If their similarity, defined as the average of equal cultural features, is bigger than a random value, then the cultural mixing takes place. The process consists of choosing one of the features presenting a difference in the culture array and agreeing on a same value.

This simple model exhibits interesting results as seen in \textbf{cite cite cite}. From a modeling perspective, the model dynamics present adaptive behavior instead of rational agents with no central authority.

We show an implementation of the basic Axelrod model using Classic DEVS in \autoref{lst:axelrod_classic}.

\begin{lstlisting}[style=base,
linewidth=\columnwidth,breaklines=true,
    basicstyle=\ttfamily\footnotesize,
    xleftmargin=2em,
    numbers=left,
    multicols=2,
    stepnumber=1,
    tabsize=2,
    firstnumber=1,
    numberstyle=\tiny,
    numberfirstline=false,
    label={lst:axelrod_classic},
    caption={Pseudocode of the Axelrod's EB-DEVS model}]
AgentState:
  neighbors_cultures = {neighbor_id: culture}
  self_culture = [randint(1, Q) for x in range(F)]

IntTransition:
  random_neighbor = random.choice(neighbors_cultures.keys())
  matching_cultures = get_matching_cultures(random_neighbor)
  share_culture = False
  if random() < matching_cultures / F:
    non_matching_cultures = get_non_matching_cultures(random_neighbor)
    random_culture, random_culture_index = random.choice(non_matching_cultures)
    self_culture[random_culture_index] = random_culture
    share_culture = True
      
ExtTransition:
  neighbors_cultures.update({neighbor_id: culture})
  
OutputFunction:
  share_self_culture_with_neighbors()
  
TimeAdvance:
  if share_culture:
    return 0
  else:
    return 1
\end{lstlisting}

\textbf{Emergence and adaptive behavior}. EB-DEVS capabilities come to life when considering the extension of the vanilla Axelrod's model. Consider the case of \textit{Fads and fashion} scenario. Fashion is defined as the cultural trait desired by many but defined by few.
It can be considered that fashion for a cultural trait is the most popular feature for any cultural trait in the agent's cultural array. This value is a macroscopic variable that can influence the cultural features at the microscopic level.

We extend the classic Axelrod model given in \autoref{lst:axelrod} in \autoref{lst:axelrod_fashion}. For this, we define a rate variable FASHION\_RATE, for which with certain probability a fashion cultural mix event is produced. This fashion cultural mix, takes a random cultural trait and copies the highest frequency value for that trait. During the internal transition, the atomic model will toss a coin to either copy a fashion feature or to behave as the classic Axelrod's model and performing a regular cultural mix.

\begin{lstlisting}[style=base,
linewidth=\columnwidth,breaklines=true,
    basicstyle=\ttfamily\footnotesize,
    xleftmargin=2em,
    numbers=left,
    multicols=2,
    stepnumber=1,
    tabsize=2,
    firstnumber=1,
    numberstyle=\tiny,
    numberfirstline=false,
    label={lst:axelrod_fashion},
    caption={Pseudocode of the Axelrod's EB-DEVS model Fads and Fashion}]
AgentState:
  neighbors_cultures = {neighbor_id: culture}
  self_culture = [randint(1, Q) for x in range(F)]

IntTransition:
  random_neighbor = random.choice(neighbors_cultures.keys())
  matching_cultures = get_matching_cultures(random_neighbor)
  share_culture = False
  do_fashion = random.random() < FASHION_RATE
  if not do_fashion and 
          random() < matching_cultures / F < 1:
    non_matching_cultures = get_non_matching_cultures(random_neighbor)
    random_culture, random_culture_index = random.choice(non_matching_cultures)
    self_culture[random_culture_index] = random_culture
    share_culture = True
  else:
    @feature, fashion = @$\color{red}v_{down}(FASHION\_FEATURE)$
    self_culture[feature] = fashion
  /*y_up = (self.state.id, self.state.culture)/*

ExtTransition:
  neighbors_cultures.update({neighbor_id: culture})
  
OutputFunction:
  share_self_culture_with_neighbors()
  
TimeAdvance:
  if share_culture:
    return 0
  else:
    return 1

CoupledState:
  models_cultures = {}

CoupledGlobalTransition(e_g, /*x_b_micro/*, @s_g_macro@):
  models_cultures.update(x_b_micro)
@  
v_down(PROPERTY):
  if PROPERTY == FASHION_FEATURE:
    mat = np.array(models_cultures.values())
    randfeature = random.randint(F)
    feature = mat[:, randfeature]
    fashion_value = np.bincount(feature).argmax()
    return randfeature, fashion_value@

\end{lstlisting}

The experiments in \autoref{fig:axelrod} were configured for a duration of 1000 time units, a F value of 5, and Q values of 5 and 20. The Q values were selected to converge into a mono cultural system and a multi cultural system respectively. We sweep the variable FASHION\_RATE from 0 to 1. If the fashion rate variable is 0, then the model behaves as the classic Axelrod model. In turn, for higher values the model presents characteristics from the fashion model, towards the value of 1, where the model is exclusively taking values from the most fashionable values on the system.

\begin{figure}[htb]
    \centering % <-- added
\begin{subfigure}{0.5\textwidth}
  \includegraphics[width=\linewidth]{imgs/axelrod__retries_10_q_5.png}
  \caption{Dissemination of culture for Q=5.}
  \label{fig:axelrod_1}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.5\textwidth}
  \includegraphics[width=\linewidth]{imgs/axelrod__retries_10_q_20.png}
  \caption{Dissemination of culture for Q=20.}
  \label{fig:axelrod_2}
\end{subfigure}

\caption{Dissemination of culture models for multiple fashion rates. Convergence to a mono cultural system (left) vs. a multi cultural system (right).}
\label{fig:axelrod}
\end{figure}

\textbf{Experimental results.} 

==> epstein.tex <==
\subsection{Sugarscape model}

\begin{itemize*}
\item In the 90's, Joshua M. Epstein and Robert Axtell presented the Sugarscape model to analyze wealth distribution in a grid of moving agents. As Schelling's model, agents move in a grid according to some rules. In this case, positions in the grid have a resource that agents consume, like sugar. Every time an agent moves, it looks for the position with the maximum amount of sugar within its range of vision, consumes all the sugar in that place and adds it up to its wealth. Immediately after this movement the agent consumes its wealth at a certain metabolic rate. If its wealth reaches zero after this consumption, then the agent dies. Each position in the grid have different sugar maximum capacity and at each time step sugar regenerates also with different rates depending on the position. 

The model have several parameters regarding the agents (like range of vision, metabolic rate and initial wealth) and the positions in the grid. For agents, the initial state is selected randomly using uniform distributions between values defined by the model parameters. (LOS RANGOS DE LAS VARIABLES??). Grid positions on the other hand are defined as a fixed terrain simulating a particular environment. In the original Sugarscape model, the grid was developed to have 2 regions with high maximum capacity, connected by a valley (middle capacity positions) and surrounded by a desert (zero capacity positions).

As is commonly known, in this model the topology of the grid is quite important for the dynamics of the simulation. Agents would prefer to move around positions with higher values and positions with less quantity of sugar would be statistically obviated. This implies an independent time step for each grid position, so we will implement them using an Atomic DEVS model independent of the moving agents.

\item Salient points related to its emergence modeling (Que encontras aca que no encontras en otro lado?)
\item Results of the original model vs original model
\item Results of the extension of model
\end{itemize*}

\begin{lstlisting}[style=base,
linewidth=\columnwidth,breaklines=true,
    basicstyle=\ttfamily\footnotesize,
    xleftmargin=2em,
    numbers=left,
    multicols=2,
    stepnumber=1,
    tabsize=2,
    firstnumber=1,
    numberstyle=\tiny,
    numberfirstline=false,
    label={lst:takahashi},
    caption={Pseudocode of the Epstein's sugarscape model. Different modeling levels are colored: Red for $V_{down}$ usage and blue for $Y_{up}$ }]
AgentState:
  position = get_initial_agent_position()
  vision = rand [1, 6]
  metabolic_rate = rand [1, 2]
  wealth = rand [5, 25]
  alive = True

AgentExternalTransition:
  return state

AgentInternalTransition:
  last_position = state.position
  /*cell_pos, cell_sugar = MAX_SUGAR_NEXT_CELL(state.position, state.vision)/*
  state.position = cell_pos
  state.wealth+= cell_sugar
  state.wealth-= state.metabolic_rate
 
  if state.wealth < 0:
      state.alive = False
  @self.y_up = (AGENT, last_position, state.position, state.alive)@
  return state

AgentOutputFunction:
  return {state.position : EMPTY}

AgentTimeAdvance:
   return reverse_exponential(0.5) if state.alive else INFINITY

CellState:
  position = INIT
  growth_rate = INIT
  sugar = INIT
  max_capacity = INIT

CellExternalTransition:
  state.sugar = 0
  return state

CellInternalTransition:
  state.sugar = state.max_capacity

  @self.y_up = (CELL, state.position, state.sugar)@

  return state

CellOutputFunction:
  return ""

CellTimeAdvance:
  return reverse_exponential(0.5)

CoupledState:
  grid = GRID(30,30)
  init_agents(50)

CoupledGlobalTransition(e_g, /*x_b_micro/*, @s_g_macro@):
  for x in /*x_b_micro/*:
    if x[0] == AGENT:
      last_pos = x[1]
      actual_pos = x[2]
      @s_g_macro.agent_grid[last_pos] = EMPTY
      s_g_macro.agent_grid[actual_pos] = OCCUPIED if x[3] else DEAD@
    elif x[0] == CELL:
      pos = x[1]
      sugar = x[2]
      @s_g_macro.sugar_grid[pos] = sugar@

\end{lstlisting}

\begin{figure}[H]
    \includegraphics[width=.45\textwidth]{imgs/epstein1.png}
    \includegraphics[width=.45\textwidth]{imgs/epstein2.png}
    \label{EPSTEINFIG}
    \caption{\textbf{Simulation and modeling of the Epstein's Sugarscape model.} Scenarios varying metabolic rate were simulated, with two different max sugar capacities: left) 4 max sugar and right) 5 max sugar points.}
\end{figure}


==> schelling.tex <==
\subsection{Schelling's segregation model (Tebi)}

In the 70's, Thomas Schelling proposed an agent based framework to model segregation. In this model, agents have assigned a color and move in a grid according to their \emph{happiness}, which is evaluated as a function of their neighbor colors. If an agent is surrounded by other agents of different color, and the number of these agents exceed a given threshold, then the agent is considered \emph{unhappy} and moves to a new random empty position in the grid. This consecutively happens with every agent in a loop until all the agents are happy. If this condition is never reached, then the simulation continues forever. Schelling used this model to simulate the formation of ghettos in the grid. The model parameters are, the size of the grid, the number of agents (colors are equally distributed) and the happiness threshold. When the simulation begins agents start to move randomly in the grid until they found a \emph{happy} position, and if they do not, agents would move forever, and the simulation does not converge.

We implemented this model in EB-DEVS as shown in Listing \ref{lst:schilling}. In the internal transition, agents do not know the grid nor the number of agents (the size of the system), they ask the environment about if they are placed in a \emph{happy} position. If so, they move to a random empty cell also provided by the environment. We utilized the upward causation / downward information features from EB-DEVS to send this information from the environment to the agents and to update the grid. The upward causation function $\delta_G$, updates the colors in the grid and the $v_{down}$ function sends the position happiness to the agents.

In this model, an emergence behaviour can be appreciated under certain conditions. As is commonly known, in the cases when system converges, ghettos appear in the grid as clusters of agents sharing the same color. System convergence depends mainly on the size of the system and the happiness threshold. This can be seen analyzing the percentage of unhappy agents as a function of time (Figure \ref{SCHELLINGFIG}). We simulated different scenarios (10 runs for each scenario) varying the happiness threshold and the size of the system. As this threshold increases the simulations took longer to finish and there is a certain limit beyond it does not converge. Also, when we changed the size of the system to less dense configurations, we obtained the same behaviour but in not converged cases, the percentage of unhappy agents reaches a different value. These differences are due to the different configuration of parameters, some of them, related to agents behavior and other to the size of the system. Now, EB-DEVS is quite useful to understand why this behaviour is emergent, because the final number of unhappy agents in a simulation, is not a direct cause of the rules of the agents, but the size of the system which is unknown by the agents.

%\item Results of the original model vs original model
%\item Results of the extension of model

\begin{lstlisting}[float,style=base,
linewidth=\columnwidth,breaklines=true,
    basicstyle=\ttfamily\footnotesize,
    xleftmargin=2em,
    numbers=left,
    multicols=2,
    stepnumber=1,
    tabsize=2,
    firstnumber=1,
    numberstyle=\tiny,
    numberfirstline=false,
    label={lst:schilling},
    caption={Pseudocode of the Schelling's segregation model. Different modeling levels are colored: Red for $V_{down}$ usage and blue for $Y_{up}$ } ]
AgentState:
  color = get_random_color(RED, GREEN)
  position = get_initial_position()
  
AgentInternalTransition:
  /*happy = coupled_model.happiness(state.position, state.color)/*
  last_pos = state.position
  if not happy:
    /*empty_cell = coupled_model.random_empty_cell()/*
    state.position = empty_cell
    @self.y_up = (last_pos, state.position)@
  return state

AgentExternalTransition:
  return state
    
AgentOutputFunction:
  return ""

AgentTimeAdvance:
   return reverse_exponential(0.5)

CoupledState:
  grid = GRID(20,20)
  init_agents(233)

CoupledGlobalTransition(e_g, /*x_b_micro/*, @s_g_macro@):
  for last_pos, actual_pos in /*x_b_micro/*:
    color_swap = @s_g_macro@.grid[last_pos]
    @s_g_macro@.grid[last_pos] = EMPTY
    @s_g_macro@.grid[actual_pos] = color_swap

\end{lstlisting}

\begin{figure}
    \includegraphics[width=.45\textwidth]{imgs/schelling1.png}
    \includegraphics[width=.45\textwidth]{imgs/schelling2.png}
    \label{SCHELLINGFIG}
    \caption{\textbf{Simulation and modeling of the Schelling's segregation model.} Scenarios varying happiness thresholds were simulated, with two different populations: left) 266 agents and right) 200 agents.}
\end{figure}

==> takahashi.tex <==

\subsection{The Takahashi's generalized exchange model}

Takahashi's global information model, is an evolutionary model where each generation
goes through a series of trials. For each trial, an agent receives a fixed number of credits that
may or may not share with a neighboring agent. The agents connection is
complete, this means that each agent can give or receive from any other agent
in the model. For each trial, an agent will choose a neighbor to give a
number of its credits.

The neighbor selection and the number of given credits are defined by two state variables.
   The giving gene (gg) defines how many credits it will give. This is an integer value between 0 and 10 (borders included).
 The tolerance gene (tg) defines how permissive it is with the neighboring altruism. Its value goes from 0.1 to 2 (borders included).
  During a trial, the agent will give to agents that have given at least \textit{tg*gg}. If there are no agents that have given such amount of credits in the previous trial it will give to the most giving agent.

Agents receive more credits than the credits given. In the case of this model agents receive twice the given amount.

After all trials finish, the evolutionary process starts removing
all agents that their amount of total credits is smaller than the mean - std.
The agents with more than mean + std credits will spawn a new generation. The ones that are between mean +/-std boundaries will remain during the next generation.

The new agents spawned into the generation has 95\% chances to remain as they were.
A small percentage will go through a mutation of their gg and tg values.

The new agents are added to the model while the number of agents is smaller than a fixed value (20 agents in accordance with the original model). Models exceeding that number are not created. New connections are made following the global model patterns.

In this model, we make use of the upward causation / downward information features from EB-DEVS and dynDEVS structural changes. The implementation is illustrated in \autoref{lst:takahashi}. The upward causation function $\delta_G$ (line 44), updates the credits that were given by agents. This captures the exchange process and allows for the $v_{down}$ (line 54) to put at disposal of the agents this information. In particular, it is used for an atomic model to select a suitable neighbor to share credits with (lines 15 and 19). The structural changes are provided by the \textit{aDEVS modelTransition} function. From the atomic model's perspective, it will trigger a \textit{modelTransition} when the number of trials for that generation are over (lines 33-34). Once the \textit{modelTransition} function returns true, the coupled model's \textit{modelTransition} function is triggered (line 65). From the coupled model's perspective, it will create, remove and reconnect the models accordingly. As there are many atomic models triggering a \textit{modelTransition} the structural changes will only be executed. This is implemented using a barrier in lines 67-68.

\begin{lstlisting}[style=base,
linewidth=\columnwidth,breaklines=true,
    basicstyle=\ttfamily\footnotesize,
    xleftmargin=2em,
    numbers=left,
    multicols=2,
    stepnumber=1,
    tabsize=2,
    firstnumber=1,
    numberstyle=\tiny,
    numberfirstline=false,
    label={lst:takahashi},
    caption={Pseudocode of the Takahashi's generalized exchange model}]

AgentState:
  gg = rand_int([0, 10])
  tg = rand([0.1, 2])
  credits = 10
  
AgentExternalTransition(received_credits):
  state.credits += RV * received_credits
  /*y_up = {'received_credits': 
    (state.id, received_credits),
    'total_credits': 
    (id, state.credits)}/*
    
AgentOutputFunction:
  suitable_neighbors = @v_down(GIVING_NEIGHBOR, state.tg * state.gg)@
  if suitable_neighbors:
    neighbor_to_give = random.choice(suitable_neighbors)
  else:
    sorted_neighbors = @v_down(NEIGHBOR_SORTED_BY_GIVER)@
    if sorted_neighbors:
        neighbor_to_give = sorted_neighbors[0]
  return neighbor_to_give

AgentInternalTransition:
  state.credits += 10
  if state.giving:
    state.credits -= state.gg
    /*y_up = {'given_credits': 
      (id, state.gg),
        'total_credits': 
      (id, state.credits)}/*

AgentModelTransition:
   return current_time % GENERATION_LENGTH

CoupledState:
  given = []
  total_credits = {}
  received_credits = {}
  given_credits = {}
  number_of_agents = TOTAL_AGENTS
  updated_agents = 0

CoupledGlobalTransition(e_g, /*x_b_micro/*, @s_g_macro@):
  for elem in x_b_micro:
    for cred_type, (agent_id, credits) in elem:
      if cred_type=='given_credits':
        state.given_credits + = credits
      if cred_type=='total_credits':
        state.total_credits[agent_id] = credits
      if cred_type=='received_credits':
        state.received_credits += credits
        
v_down(PROPERTY, parameter):
  if PROPERTY == TOTAL_CREDITS_MEAN:
    return mean(state.total_credits.values())
  if PROPERTY == GIVING_NEIGHBOR:
    bigger_than = parameter
    givers = [model_id for model_id, given_creds in given_credits.values() if given_creds >= bigger_than]
    return givers
  if PROPERTY == NEIGHBOR_SORTED_BY_GIVER:
     return [el[0] for el in sorted(given_credits.items(),
                key= lambda x: x[1], reverse=True)]
        
CoupledModelTransition():
  state.updated_agents +=1
  if state.updated_agents==state.number_of_agents
      g_mean = @v_down[TOTAL_CREDITS_MEAN]@
      g_sd = @v_down[TOTAL_CREDITS_MEAN]@
    
      to_duplicate = [model_id for model_id, model_credits in total_credits.keys() if model_credits > (g_mean + g_sd)]
      to_eliminate = [model_id for model_id, model_credits in total_credits.keys() if model_credits < (g_mean - g_sd)]

    for agent in to_eliminate:
      remove(agent)
      
    for agent in to_duplicate:
      add_agent()
      if state.number_of_agents >= TOTAL_AGENTS:
        break

    reconnect_agents()
    updated_agents = 0
\end{lstlisting}


\begin{figure}[h]
\caption{Takahashi's exchange}
\centering
\includegraphics[width=0.95\textwidth]{imgs/takahashi_retries_5.png}
\end{figure}


\begin{itemize*}
\item Introduction to the model
\item Salient points related to its emergence modeling (Que encontras aca que no encontras en otro lado?)
\item Results of the original model vs original model
\item Results of the extension of model
\end{itemize*}

